Reachability and Top-k Reachability Queries with Transfer Decay

The prevalence of location tracking systems has resulted in large volumes of spatiotemporal data generated every day. Addressing reachability queries on such datasets is important for a wide range of applications (surveillance, public health, social networks, etc.) A spatiotemporal reachability query identifies whether a physical item (or information etc.) could have been transferred from the source object $O_S$ to the target object $O_T$ during a time interval $I$ (either directly, or through a chain of intermediate transfers). In previous research on spatiotemporal reachability queries, the number of such transfers is not limited, and the weight of a piece of transferred information remains the same. This paper introduces novel reachability queries, which assume a scenario of information decay. Such queries arise when the value of information that travels through the chain of intermediate objects decreases with each transfer. To address such queries efficiently over large spatiotemporal datasets, we introduce the RICCdecay algorithm. Further, the decay scenario leads to an important extension: if there are many different sources of information, the aggregate value of information an object can obtain varies. As a result, we introduce a top-k reachability problem, identifying the k objects with the highest accumulated information. We also present the RICCtopK algorithm that can efficiently compute top-k reachability with transfer decay queries. An experimental evaluation shows the efficiency of the proposed algorithms over previous approaches.

==> text/abstract.tex <==
\section*{Abstract}
\label{sec:abstract}


The prevalence of location tracking systems has resulted in large volumes of spatiotemporal data generated every day. Addressing reachability queries on such datasets is important for a wide range of applications, such as security monitoring, surveillance, public health, epidemiology, social networks, etc. A spatiotemporal reachability query identifies whether a physical item (or information etc.) could have been transferred from the sourse object $O_S$ to the target object $O_T$ during a time interval $I$ (either directly, or through a chain of intermediate transfers). In previous research on spatiotemporal reachability queries, the number of such transfers is not limited, and the weight of a piece of transferred information remains the same.
This paper introduces novel reachability queries, which assume a scenario of \textit{information decay}. Such queries arise when the value of information that travels through the chain of intermediate objects \textit{decreases} with each transfer. This in turn leads to an interesting \textit{extension}: if there are many different sources of information, the aggregate value of information an object can obtain varies. As a result, under the decay scenario, we introduce a top-\textit{k} reachability problem, identifying the \textit{k} objects with the highest accumulated information. We design two algorithms: RICCdecay and RICCtopK that can efficiently compute reachability with transfer decay queries and top-k queries respectively on large spatiotemporal datasets.
\vspace{-0.2in}
%Several variation on spatiotemporal reachability queries are studied in. 

 
%Next, we formulate/restate/remind the definition of a meeting as in Chapter 2: Two objects, $O_i$ and $O_j$, had a {\em meeting} during the time interval $I_m = [\tau_{s}, \tau_{f}]$, if they had been within the threshold distance $d_{cont}$ from each other at each time instant $\tau_{k} \in [\tau_{s}, \tau_{f}]$. Such a meeting is denoted $<O_i, O_j, I_m>$.  The {\em duration} of this meeting is $m = \tau_{f} - \tau_{s} $. 

%In the last work, to complete the transfer, the objects are required to stay within the contact distance for a particular time interval, which is named a {\em required meeting duration} and denoted as $m_q$. 
%In general, $m_q$ may vary from one query to another depending on the transfer scenario.Also, the required meeting duration may be different from the actual meeting duration. 





==> text/description.tex <==
\section{Answering Reachability Queries with Transfer Decay}
\label{sec:problemDescriptionCh4}


Given two objects $O_S$ and $O_T$, and a time interval $I$, a spatiotemporal reachability query identifies whether information (or physical item etc.) could have been transferred from $O_S$ to $O_T$ during $I$ (typically indirectly through a chain of intermediate transfers). In the previous research on spatiotemporal reachability queries~\cite{Shahabi, ricc, RICCmeet}, the number of such transfers is not limited, and the weight of a piece of transfered information remains the same. Each of these works introduces a different reachability scenario. In ~\cite{Shahabi}, it is assumed that information can be passed from one object to another instantaneously, while ~\cite{ricc, RICCmeet} consider the problems of reachability with processing and transfer delays (or meetings)  respectively. 

%Several variation on spatiotemporal reachability queries are studied in. 

 
%Next, we formulate/restate/remind the definition of a meeting as in Chapter 2: Two objects, $O_i$ and $O_j$, had a {\em meeting} during the time interval $I_m = [\tau_{s}, \tau_{f}]$, if they had been within the threshold distance $d_{cont}$ from each other at each time instant $\tau_{k} \in [\tau_{s}, \tau_{f}]$. Such a meeting is denoted $<O_i, O_j, I_m>$.  The {\em duration} of this meeting is $m = \tau_{f} - \tau_{s} $. 

In the last work, to complete the transfer, the objects are required to stay within the contact distance for a particular time interval, which is named a {\em required meeting duration} and denoted as $m_q$. 
%In general, $m_q$ may vary from one query to another depending on the transfer scenario.Also, the required meeting duration may be different from the actual meeting duration. 




However, even if a meeting between $O_S$ and some object $O_i$ was long enough to satisfy the $m_q$ requirement, under some circumstances, the transfer may fail to occur or the value of the transferred item may go down (e.g., a signal loss during the communication). To account for such events, we introduce a new type of queries, namely {\em reachability queries with transfer decay}. Let $d$ denote a {\em transfer decay} - a part of information lost during one transfer ($d \in (0, 1)$). Then $p = 1 - d$ ($p \in (0, 1)$) will define the part of the transfered information.
Suppose, a weight of the item carried by a source object $O_S$ is $w$. Then, during a valid meeting, $O_S$ can transfer this item to $O_i$, however, considering the decay, the value of information, obtained by $O_i$ will lessen, and become $wp$.  
%and calculate a weight of the information transferred to $O_i$ as $wp$. 
With each further exchange, the value of a received item will continue to decrease. This process can be modeled with an exponential decay function. Let function $\tilde f_w(O_i^{(\tau_j)})$ compute the weight of an item acquired by object $O_i$ by the time $\tau_j$. Then, assuming that the transfer decay $d$ and thus $p$ are constant for the same item or piece of information, $\tilde f_w(O_i^{(\tau_j)}) = wp^h$, where $h$ is the minimum number of transfers (or hops) that the item had to travel through from the source $O_s$ before reaching object $O_i$.

%Consider the example in Figure ????  
%~\ref{name}.
%The graph (Figure ???? (a)) shows the meeting between the objects $O_1, O_2, O_3, O_4,$ and $O_5$ during the time interval $I = [\tau_0; \tau_6????]$. For this example, it is assumed that $O_1$ is the source object, and $p = 0.8$. The values for $f_w(O_i^{(\tau_j)})$ are computed for each object at each time instant and recorded in the table on the right (Figure ???? (b)). 
Note, that the scenario with $p = 1$ corresponds to the reachability with transfer delays problem described in{~\cite{RICCmeet}}.

If $p < 1$, with each transfer the value of $wp^h$ decreases exponentially. After a number of transfers, it may becomes too small, and the user may decide to disregard it. For this purpose, we introduce a weight function $ f_w(O_i^{(\tau_j)})$ and a {\em threshold weight of transfer} $\nu$ ($\nu \in [0, 1) $):  

\begin{equation}
f_w(O_i^{(\tau_j)}) =  \begin{cases}
\tilde f_w(O_i^{(\tau_j)}),  & \text{if $ wp^h \geq \nu$ }\\
0, & \text{otherwise}\\
\end{cases}
\end{equation}

The reachability problem with meetings and transfer decays, will be named {\em (m, d)-reachability}.
Object $O_T$ is considered to be  {\em (m, d)-reachable} from object $O_S$ during time interval $I = [\tau'_s, \tau'_f]$ if there exists a chain of subsequent meetings $<O_S, O_{i_1}, I_{m_0}, f_w(O_{i_1})>$, $<O_{i_1}, O_{i_2}, I_{m_1}, f_w(O_{i_2})>$, ... ,$<O_{i_k}, O_T, I_{m_k},  f_w(O_{i_T})>$, where (i) each $I_{m_j} = [\tau_{s_j}, \tau_{f_j}]$ is such that $\tau_{f_j} -\tau_{s_j} \geq m_q$, $\tau'_s \leq \tau_{s_0}$, $\tau_{f_k} \leq \tau'_f$, and $\tau_{s_{j+1}} \geq \tau_{s_j}$ for $j= 0, 1, ..., k-1$, and (ii) each  $f_w(O_{i_j}) > 0$.

We assume that the values of $d$ and $\nu$ are query specified. 
An {\em (m, d)-reachability} query $Q_{mp}$: $\{O_S, O_T, I, m_q, d, \nu\}$ determines whether object $O_T$ (target) is reachable from object $O_S$ (source) during time interval $I = [\tau_s, \tau_f]$, given required meeting duration $m_q$, transfer decay $d$, and threshold probability of transfer $\nu$, and reports the earliest time instant when $O_T$ was reached.

In our work, we design algorithm RICCdecay that can efficiently compute (m, d)-reachability queries on large spatiotemporal datasets. It consists of two stages, preprocessing and query processing. During the preprocessing stage, RICCdecay precomputes all meetings, as well as reachability between the objects on short time intervals. For the reachability, for each object $O_j$ that can be reached from object $O_i$, the algorithm also finds the minimum number of transfers that $O_j$ can be reached in. Later, an index structure, similar to the one designed for the RICC algorithm~\cite{ricc} is constructed. 


